Unilateral Antidotes to DNS Cache Poisoning

We investigate defenses against DNS cache poisoning focusing on mechanisms that can be readily deployed unilaterally by the resolving organisation, preferably in a single gateway or a proxy. DNS poisoning is (still) a major threat to Internet security; determined spoofing attackers are often able to circumvent currently deployed antidotes such as port randomisation. The adoption of DNSSEC, which would foil DNS poisoning, remains a long-term challenge. We discuss limitations of the prominent resolver-only defenses, mainly port and IP randomisation, 0x20 encoding and birthday protection. We then present two new (unilateral) defenses: the sandwich antidote and the NAT antidote. The defenses are simple, effective and efficient, and can be implemented in a gateway connecting the resolver to the Internet. The sandwich antidote is composed of two phases: poisoning-attack detection and then prevention. The NAT antidote adds entropy to DNS requests by switching the resolver's IP address to a random address (belonging to the same autonomous system). Finally, we show how to implement the birthday protection mechanism in the gateway, thus allowing to restrict the number of DNS requests with the same query to 1 even when the resolver does not support this.

==> antidotes.tex <==
\section{Proposed Antidotes to DNS Poisoning} \label{s:proposed}
In this section we briefly review proposed anti-poisoning defenses against spoofers, that require integration on the side of the local DNS resolver only. These techniques can be broadly categorised as follows: (1) mechanisms that increase entropy in DNS packets (subsection \ref{sc:entropy}), and (2) mechanisms that inspect the DNS responses to detect forgery (subsection \ref{ss:anax}). %We dedicated a subsection to 0x20 due to its importance, and since we discuss some issues and suggest improvements. 

\subsection{Entropy Increasing Mechanisms}\label{sc:entropy}
Unilateral entropy increasing mechanisms, most notably: source port randomisation (SPR) \cite{Bernstein:DNS}, source/destination IP address randomisation (IPR) and DNS 0x20 encoding \cite{DagonAVJL08}, add more randomness to DNS packets, in order to make it more difficult for the spoofing adversary to craft a valid DNS response, that would get accepted {\em and} cached by the local DNS resolver. %Entropy increasing mechanisms received a lot of attention from the research community, were scrutinised and some of them became widely deployed.
%Entropy increasing mechanisms do not inspect DNS packets to identify forgery attacks, but merely use random values in several fields of the DNS packets, and validate the same values in DNS responses. 
In order to produce a successful forgery the attacker has to guess {\em all} the values in the validation fields correctly. The more random values pertain in the DNS requests, the lower the probability of the attacker to produce a successful guess. Entropy increasing mechanisms do not try to identify forgery attacks and respond to them, but attempt to increase the difficulty of producing a successful forgery.

Unfortunately, the number of fields in the DNS packet, that could be used to add randomness, is limited: the transaction ID field in the DNS packet, the source port, source/destination IP addresses, and the choice of upper/lower case for the query (since DNS is case-insensitive; this is the field used by DNS 0x20 encoding). % In particular, the DNS is still vulnerable to DNS poisoning attacks by spoofing adversaries. 
%We next review the notion of entropy, and then discuss the deficiencies inherent in each technique.
\ignore{
\subsubsection{Entropy in DNS Packets}
Entropy, with respect to our subject, measures the amount of uncertainty (i.e., randomness) contained in DNS packets. There are many recommended techniques for adding entropy using the validation fields, e.g., source port randomisation, and when issuing the DNS request, the resolver should select the validation fields at random. Upon receipt of a DNS response the resolver should then verify that the same values appear in DNS response, and otherwise ignore the response. 

For a poisoning attack to succeed the attacker has to craft a DNS response with validation fields that match those in DNS request, such that the malicious DNS response arrives before the authentic response sent by the authority DNS server. Since a spoofing attacker cannot predict the values of the validation fields (those were selected at random by the DNS resolver) it has to: either (1) attempt to guess or (2) perform a brute force attack, i.e., generate a sequence of DNS responses trying all possible combinations of the values in validation fields; see \cite{rfc5452} for a calculation of the probabilities involved.
} % ignored: imho, this just repeats above. 

\ignore{
\subsubsection{Entropy Increasing Mechanisms: Shortcomings}
Transaction ID alone does not provide protection and if additional countermeasures are not employed, DNS resolver can be poisoned within seconds. Indeed \cite{Bernstein:DNS} suggested already in 2002 to randomise also the source ports. Source port randomisation can add up to $16$ additional bits of randomness. However, network address translation (NAT) devices are known to ruin source port randomisation, and local DNS resolvers located behind NAT devices, which is the typical case, cannot rely on source port randomisation. In addition, source port randomisation alone (along with random transaction ID), does not provide sufficient protection and poisoning the cache is still possible. NAT devices also ruin source IP address randomisation, as they modify the IP in outbound packets to their own. Furthermore, DNS servers are often allocated at most $5$ additional IP addresses, which clearly does not add significant randomness to DNS packets, but only increases the search space by at most a factor of $2^5$.
}
\subsubsection{Port Randomisation}
%most resolvers were patched to send the DNS queries from random source ports.
%\begin{wrapfigure}{r}{0cm}
Following to Kaminsky attack, \cite{Kaminsky08}, the need to patch the DNS resolvers to send DNS requests from random ports became apparent. Using random source ports adds another $16$ bits of entropy, resulting in a search space of $2^{16}\times 2^{16}=2^{34}$ bits, which makes successful poisoning significantly more difficult to achieve.\\\indent 
Unfortunately, source port randomisation (SPR) is resource intensive, and as noted in \cite{DagonADLLL09,DV} may be inappropriate for busy DNS servers or embedded devices. In addition, as pointed out by \cite{DagonAVJL08}, determined attackers can overcome source port randomisation, by sending large amounts of traffic, e.g., from many zombie computers, thus covering all the search space and eventually producing a valid DNS response. Therefore, enhancing DNS security using SPR and transaction ID alone may not suffice.\\\indent
 %Furthermore, as we show in \cite{nat:atk}, source port randomisation can be circumvented when local DNS resolver is located behind a firewall or a NAT device.
Furthermore, many (or most) DNS resolvers are located behind NAT devices, and as \cite{Cross08,VU800113} noted, NAT devices that use sequential assignment of external ports, may expose (even the patched) local DNS resolvers, to poisoning attacks, since NAT could reduce source port randomisation implemented by the local resolvers.

\subsubsection{IP Randomisation}
IP addresses are known to be a scarce resource on the Internet. IP address is composed of $32$ bits, resulting in at most $2^{32}$ possible addresses. Due to this shortcoming, the DNS resolvers are often allocated a single IP address, and authority DNS servers are allocated at most $3$ IP addresses. This can increase the search space of the attacker by at most a factor of $1\times 3$, which does not offer sufficient protection. In addition, the DNS resolvers that are located behind NAT devices, which is the typical case, lose the IP randomisation, even if they are allocated several IP addresses.

\subsubsection{DNS 0x20 Encoding}\label{sc:0x20}%is currently in the process of standartisation. 
Dagon {\em et al.}~\cite{DagonAVJL08} present an innovative technique, 0x20-encoding, for improving DNS defense by increasing entropy of DNS queries against poisoning by spoofed responses. The technique is based on an observation that domain names are case insensitive, however, most authoritative servers copy the string of the domain name from the incoming request to the response they send back, {\em exactly} as sent - preserving the case of each letter. They suggest to randomly toggle the case of letters of which the domain name consists, and validate them in response. If the domain name $d$ contains $l(d)$ alphabetic characters, this increases the space of identifiers by factor of $X(d)=2^{l(d)}$, e.g., $X(\textsc{www.google.com})=2^{12}$ and $X(\textsc{a9.com})=2^4$. 

Note that in Kaminsky-style attacks, the query is for a non-existing domain name chosen by the attacker, e.g., to poison addresses in the domain {\sc google.com}, an attacker may issue a query for $r${\sc .google.com} where $r\in_R\{0,\ldots,9\}^8$ is a random string of $8$ digits, resulting in a domain name with only $9$ letters, i.e., factor of only $X=2^9$; namely, 0x20 encoding is less effective for domain names containing few letters - which are often the most important domains, e.g., the Top Level Domains (TLDs) such as {\sc .com} and {\sc .uk}. 

Although 0x20 encoding, as presented by Dagon {\em et al.}, introduces significant extra entropy to DNS requests, an attacker may still be able to poison `high value' domain names with a rather small factor of poisoned responses. Therefore, there is need in alternative or additional technique to protect the TLDs and other domain names containing only few letters, e.g., {\sc a9.com}. 

% Note that, when considering hierarchical structure of the DNS resolvers, as in Figure~\ref{dns:hie}, for the defense mechanism to be useful, the resolvers have to either preserve the case of the DNS query, or support 0x20 encoding technique. However, if attacker succeeds in poisoning the name server's record in the proxy resolver, the DNS queries, of resolvers lower in hierarchy, will go to the attacker's server.

%We note that the 0x20 encoding technique is not supported by all DNS resolvers, e.g., Unbound. %~\cite{}, w
%When the DNS resolver, e.g., of some organisation, is located behind a higher level resolver, e.g., that of ISP\footnote{This is typically the case in many subnets, where the local DNS resolvers, lower in hierarchy use higher layer resolvers as forwarders.}. 
%Specifically, when a lower layer DNS resolver, that implements the 0x20 encoding, sends the DNS queries via its ISP's DNS resolver (that does not support 0x20), the DNS queries in the responses will not maintain the case that was originally set by the lower layer resolver, and query will fail.
\ignore{
\subsubsection{Poisoning ``high-value'' Domain Names} 
Dagon {\em et al.}~\cite{DagonAVJL08} %noted, that the impact of 0x20 encoding on the effort required to spoof a specific domain name, is a function of the number $l$ of 0x20 characters in the domain name. They 
found that for many (or most) domains $d$ in queries, $l(d)\geq 12$, hence resulting in a factor of $X(d)\geq 2^{12}$ in the number of spoofed responses that the attacker must send in order to poison the domain name.\\\indent
Unfortunately, this argument is slightly flawed: we must always assume that an attack will happen at the weakest part of the defense. In this case, in order to poison a particular FQDN, say {\sc www.google.com} (containing exactly the `typical' 12 letters), the attacker may prefer not to send poisoned responses to a query for {\sc www.google.com}; instead, it would poison {\sc www.google.com} by poisoning the domain of the name server. Namely, the attacker may send a query to the domain name {\sc 666.google.com} (containing only 9 letters), and thereby poison the NS record of domain {\sc google.com}, or the A record of the name server of {\sc google.com} (or directly poison the A record of {\sc www.google.com}). Furthermore, the attacker may even prefer to send a query to {\sc 666666.com}, containing only three letters, and thereby poison the TLD name server of {\sc .com} domain (and through it, easily poison {\sc www.google.com} as well as any other {\sc .com} subdomain).\\\indent
In fact, in Kaminsky-style attacks, the query is intentionally for a non-existing domain name chosen by the attacker, e.g., to poison addresses in the domain {\sc google.com}, an attacker may perform query for $r${\sc .google.com} where $r\in_R\{0,\ldots,9\}^8$ is a random string of $8$ digits, resulting domain name with only $9$ letters, i.e., factor of only $X=2^9$. Namely, 0x20 encoding is less effective for domain names containing few letters - which are often the most important domains, e.g., the Top Level Domains (TLDs) such as {\sc .com} and {\sc .uk}. Therefore, there is need in another technique to protect the TLDs and other domain names containing only few letters, e.g., {\sc a9.com}, and to protect any domain against poisoning of the TLD or other high-level domain containing only few letters.\\\indent
We therefore conclude that although 0x20 encoding, as presented by  Dagon {\em et al.} \cite{DagonAVJL08}, provides significant extra entropy, % only to queries to `typical high value' domain names, but 
 an attacker may still be able to poison `high value' domain names with a rather small factor (e.g., 8) of poisoned responses.\\\indent
In the following subsection, we fix this issue, by presenting simple improvements to the 0x20 encoding technique, thus allowing to ensure significant entropy even to domain names containing only few 0x20 characters.   

\subsubsection{Adding Entropy to Short DNS Queries}
Following to our observation above, we next present few simple ideas, that can  significantly improve the protection afforded by 0x20-encoding for TLDs and other domain names containing only few letters.\\\indent% (hence not well protected by 0x20 encoding). 
We first consider the most typical case of queries with very short domain names: queries to a root name server for the address of a TLD name server $z$, or to a TLD name server for the address of the name server $y.z$.\\\indent
Our solution to this case is similar to some of the ideas in the WSEC DNS proposal \cite{DBLP:conf/dsn/PerdisciALL09}. Namely, suppose a resolver has to make such a query, say to the TLD $z$ with the query $\phi=y.z$ or $\phi=x.y.z$, where $\phi$ contains only few letters. We notice that regardless of the value (or existence) of the subdomain $x$, the response to the query should always supply only identification of the name server of domain $y.z$, by providing NS resource record, and usually also the corresponding A resource record, as a `glue'. Hence, the resolver can simply issue an alternative query to the domain $r.y.z$, where $r$ is a random string containing 0x20 characters, of sufficient length.
%Specifically, in contrast to the proposal in \cite{DBLP:conf/dsn/PerdisciALL09}, 
We suggest that the prefix $r$ were a fixed, sufficiently long, reserved string, e.g., %{\sc Randomisation} (13 letters) or 
{\sc FixedRandomisationString} (24 letters). As a result, the query string will contain a sufficient number of alphabetic characters thus contributing to the amount of entropy that could be used for 0x20 encoding. %, to prevent poisoning using 0x20 encoding (`case toggling'). 
Since the requested domain is a subdomain of $y.z$, the response will contain the NS and IP address for the name server for  $y.z$, as required.
Prepending a fixed string, as above, has an advantage over the use of a purely random string, as in WSEC DNS \cite{DBLP:conf/dsn/PerdisciALL09}, since requests with fixed strings as a subdomain would work well with possible caching by `higher level' resolvers (such 0x20 encoding supports caching).\\\indent % Note that this technique works well, even if both the TLD $z$ and the entire domain $y.z$ do not contain 0x20 characters at all (although, in fact, all current TLDs consist of at least two letters).\\\indent
However, this technique cannot be applied if the request is for the IP address ({\sc A} record) of some FQDN $x.y.z$ containing insufficient number of letters, and it is sent to the name server of domain $y.z$ (rather than a request for the address of the name server for $y.z$). For example, assume that the attacker is sending a request for, say {\sc 666.google.com}, which contains only nine letters, and sends a response containing a poisoned NS record for the zone {\sc google.com} (or a poisoned A record for the name server, e.g., {\sc ns.google.com}). This threat is a bit lower than that of poisoning the TLD name servers; however, we can provide some solutions for this case as well.\\\indent
The best solution requires minimal effort from the manager of the zone (i.e., maintaining the authoritative name server for the zone $y.z$, e.g., for {\sc google.com}). Specifically, the manager can publish a policy, stating that his zone contains only FQDNs with at least a given number of letters. If shorter domain names are necessary, e.g., for user-friendliness or marketing considerations, they can be mapped by a {\em fixed} {\sc CNAME} record\footnote{The {\sf cname} RR has to be fixed, e.g., {\sf FixedRandomisationString}$.x.y.z$ to prevent the attacker from sending the {\sf cname} RR of its choosing.} to a longer alias (i.e., the policy allows FQDNs with few 0x20 characters, however would always return a CNAME record mapping to an alias with sufficient number of 0x20 characters).
Domains should signal their adherence to this policy, e.g., by a policy record kept in some fixed location, e.g., {\sc MinimalFQDNlengthPolicy.$y.z$}. This would require a very minor modification, only to the owners of such `short' domain names $x$.
}
\subsection{Forgery Detection Mechanisms}\label{ss:anax}
% The prominent anti-poisoning techniques discussed above increase the difficulty of successful poisoning and reduce the success probability by introducing additional sources of randomness, e.g., selecting the source port for each outgoing DNS request at random. In particular, these techniques do not observe the incoming DNS responses, e.g., to identify a suspicious IP address of the requested domain, and thus do not introduce additional processing or delay. The other category, which we focus on in this section, attempts to detect forged DNS responses by observing the payload and analysing the authenticity using an auxiliary information. Auxiliary information can be based on DNS responses obtained from other peers, i.e., `the collaborative approach', or by applying techniques from machine learning. %e.g., \cite{park2004codns,poole2006confidns,yuan2006dox,sun2009dependns}, 
The `forgery detection' mechanisms follow two approaches: the collaborative approach and techniques from machine learning.
According to the collaborative approach the authenticity of a DNS response is validated by distributing the DNS requests across hosts in the system, e.g., \cite{park2004codns,poole2006confidns,sun2009dependns}, or by consulting a set of trusted peers, \cite{yuan2006dox}, and then, e.g., taking the majority answer. 
CoDNS, ConfiDNS and DoX, \cite{park2004codns,poole2006confidns,yuan2006dox}, send the requests to several peers in a peer-to-peer network and accept the first DNS response; if the first response is forged, it is still accepted.
 DepenDNS, \cite{sun2009dependns}, queries several DNS resolvers, and accepts the DNS response of the majority. DepenDNS relies on open recursive DNS resolvers to obtain DNS responses; open recursion DNS services are known to expose DNS to attacks. Furthermore, recently, \cite{alfardan2011analysis} showed that DepenDNS does not protect DNS against poisoning attacks. % CoDNS, ConfiDNS, DepenDNS, DoX,
%e.g., by comparing it with other DNS responses and taking the majority answer (2). In fact, the collaborative approachOne of the approaches to validate authenticity of a DNS response is by consulting the peers. 
The common shortcomings of the collaborative approach are most notably the performance penalty, i.e., additional processing and communication delays, that they introduce to every DNS request, even when the system is {\em not} under attack, and the significant infrastructure that is required for deployment. In addition, techniques that are based on distributing the DNS request to several nodes, e.g., \cite{park2004codns}, are also exposed to cache poisoning attacks, as the first DNS response that arrives is accepted. \\\indent 
% The idea behind Cooperative DNS resolution systems, e.g., CoDNS, and ConfiDNS, \cite{park2004codns,poole2006confidns}
% DoX~\cite{yuan2006dox} uses a peer-to-peer network to validate DNS resource records and requires significant infrastructure for deployment.
% Instead of querying a single resolver, DepenDNS~\cite{sun2009dependns} replicates the query and sends it to multiple resolvers; then it selects the response from the DNS messages that it receives according to an algorithm.
A recent technique, by Antonakakis {\em et al}~\cite{antonakakis2011centralized}, employs mechanisms from machine learning to identify suspicious IP addresses. Specifically, \cite{antonakakis2011centralized} designed a centralised poisoning detection system called Anax, which is based on the observation that DNS records direct users to a known set of NS records, while poisoned records redirect users to new IP addresses, outside of the victim's address space.
%Anax is based on an assumption that as a result of Kaminsky attack, the poisoned resource records will direct the hosts to an authoritative name server outside of the victim's address space. Anax is an alternative centralised DNS design, which periodically sends resolution requests via different local DNS resolvers, 
However, deployment requires trust in one central entity that should be consulted to establish authenticity of the DNS responses. In addition, this mechanism also introduces delays and may have false positives, e.g., if an authority DNS server was moved to a new IP address for load distribution.

\ignore{
\subsection{The Best of both Worlds}
Both categories, the increasing entropy (Section~\ref{sc:entropy}) and the forgery detection (Section~\ref{ss:anax}) mechanisms, have different shortcomings and most importantly`: the DNS cache poisoning problem is not yet solved. Our central contribution, in Section~\ref{sc:res:fw}, is a technique based on a combination of the advantages of both categories. Specifically, the mechanism, coined the {\em sandwich antidote}, is only activated when the forgery attempt is detected, then, additional entropy is added to DNS packets, by issuing DNS requests for a non-existent hostname, i.e., by prepending a random string to the domain name, following the WSEC idea in~\cite{DBLP:conf/dsn/PerdisciALL09}, and sending the request for the original DNS query between those two. The random string increases the entropy in DNS request, making it impossible for the attacker to craft a valid DNS response. The responses are accepted if they are correct, and arrive in the same order in which they were sent. Details in Section~\ref{sc:res:fw}.
} % end ignore

==> conc.tex <==
\section{Conclusions}\label{sc:conc}
Currently, many DNS resolvers are still vulnerable to DNS poisoning attacks by determined adversaries, only requiring from them the ability to spoof packets. DNS poisoning can be used for a wide range of devastating attacks, hence, it is essential to develop interim solutions, to ensure security until the long-term cryptographic DNS-security mechanisms are widely deployed. Preferably, such interim antidotes to DNS poisoning should require changes only in the resolver, or, better yet, only in the gateway connecting the resolver to the Internet. 

We investigated unilateral defenses against the DNS cache poisoning by spoofing adversaries, and presented new and improved mechanisms. Our central contribution is the {\em sandwich antidote} to DNS poisoning, which operates in two phases: detecting and then preventing poisoning attacks. We also presented the {\em NAT antidote}, which enhances DNS security by increasing the entropy in DNS packets for most subnets by a factor of $2^{11}$, by picking a random source IP address from a pool of addresses available to the organisation. These solutions can be easily deployed in gateways (we present proof of concept code), to provide immediate defense against DNS poisoning. 

% 
% We discuss the advantages and shortcomings of the existing techniques against spoofers, and enhance DNS resistance to poisoning using two  and present the {\em sandwich antidote} that to DNS cache poisoning by spoofing adversaries.   investigate unilateral anti-spoofing defenses, requiring modifications to local DNS resolver only. We present two anti-poisoning defenses: Discard Forgery, requiring modifications to local resolver only, and SOA Randomisation, requiring modifications to SOA DNS. We also initiate a new research direction, investigating solutions against DNS poisoning in firewalls, and present Linux firewall-based implementations. We analyse the effectiveness of anti-poisoning defense techniques (investigated in this work) against spoofing adversaries, specifically, Discard forgery, SoaR, source port randomisation, DNS 0x20 encoding, and suggest to combine them together for best protection. We also suggest ways to enhance security of DNS 0x20 encoding for TLD and short domains.
% 
% Finally, we present several open research directions, based on our proposed solutions. Specifically, we encourage investigating other variations of Discard forgery, and to develop kernel based implementations. We implemented SoaR defense in firewall, and suggest to extend the implementation to SOA DNS.

